Audio-driven Neural Gesture Reenactment with Video Motion Graphs

Human speech is often accompanied by body gestures including arm and hand gestures. We present a method that reenacts a high-quality video with gestures matching a target speech audio. The key idea of our method is to split and re-assemble clips from a reference video through a novel video motion graph encoding valid transitions between clips. To seamlessly connect different clips in the reenactment, we propose a pose-aware video blending network which synthesizes video frames around the stitched frames between two clips. Moreover, we developed an audio-based gesture searching algorithm to find the optimal order of the reenacted frames. Our system generates reenactments that are consistent with both the audio rhythms and the speech content. We evaluate our synthesized video quality quantitatively, qualitatively, and with user studies, demonstrating that our method produces videos of much higher quality and consistency with the target audio compared to previous work and baselines.

==> LaTeX/sections/training.tex <==

\begingroup
\setlength{\tabcolsep}{1pt} % Default value: 6pt
\begin{table*}
\begin{center}
\begin{tabular}{c c c c c c}
\includegraphics[width=0.16\linewidth]{LaTeX/imgs/image_interpolation/dave02_in0.jpg} &
\includegraphics[width=0.16\linewidth]{LaTeX/imgs/image_interpolation/dave02_ff_rec.jpg} &
\includegraphics[width=0.16\linewidth]{LaTeX/imgs/image_interpolation/dave02_slm_rec.jpg} &
\includegraphics[width=0.16\linewidth]{LaTeX/imgs/image_interpolation/dave02_vnet_rec.jpg} &
\includegraphics[width=0.16\linewidth]{LaTeX/imgs/image_interpolation/dave02_ebd_rec.jpg} &
\includegraphics[width=0.16\linewidth]{LaTeX/imgs/image_interpolation/dave02_ours_rec.jpg} \\


\includegraphics[width=0.16\linewidth]{LaTeX/imgs/image_interpolation/dave02_in1.jpg} &
\includegraphics[height=0.16\linewidth]{LaTeX/imgs/image_interpolation/dave02_ff_zoom.jpg} &
\includegraphics[height=0.16\linewidth]{LaTeX/imgs/image_interpolation/dave02_slm_zoom.jpg} &
\includegraphics[height=0.16\linewidth]{LaTeX/imgs/image_interpolation/dave02_vnet_zoom.jpg} &
\includegraphics[height=0.16\linewidth]{LaTeX/imgs/image_interpolation/dave02_ebd_zoom.jpg} &
\includegraphics[height=0.16\linewidth]{LaTeX/imgs/image_interpolation/dave02_ours_zoom.jpg} \\

 & & & & & \\[-0.5em]

\includegraphics[width=0.16\linewidth]{LaTeX/imgs/image_interpolation/jun_in0.jpg} &
\includegraphics[width=0.16\linewidth]{LaTeX/imgs/image_interpolation/jun_ff_rec.jpg} &
\includegraphics[width=0.16\linewidth]{LaTeX/imgs/image_interpolation/jun_slm_rec.jpg} &
\includegraphics[width=0.16\linewidth]{LaTeX/imgs/image_interpolation/jun_vnet_rec.jpg} &
\includegraphics[width=0.16\linewidth]{LaTeX/imgs/image_interpolation/jun_ebd_rec.jpg} &
\includegraphics[width=0.16\linewidth]{LaTeX/imgs/image_interpolation/jun_ours_rec.jpg} \\

\includegraphics[width=0.16\linewidth]{LaTeX/imgs/image_interpolation/jun_in1.jpg} &
\includegraphics[width=0.16\linewidth]{LaTeX/imgs/image_interpolation/jun_ff_zoom.jpg}  &
\includegraphics[width=0.16\linewidth]{LaTeX/imgs/image_interpolation/jun_slm_zoom.jpg} &
\includegraphics[width=0.16\linewidth]{LaTeX/imgs/image_interpolation/jun_vnet_zoom.jpg} &
\includegraphics[width=0.16\linewidth]{LaTeX/imgs/image_interpolation/jun_ebd_zoom.jpg} &
\includegraphics[width=0.16\linewidth]{LaTeX/imgs/image_interpolation/jun_ours_zoom.jpg} \\
2 Input Frames &
 FeatureFlow\cite{gui2020featureflow} & SuperSlMo\cite{jiang2018super} & vUnet\cite{esser2018variational} & EBDance\cite{chan2019dance} & Ours\\
\end{tabular}
\end{center}
\captionof{figure}{Comparison of frame interpolation results.}
\label{fig:interpolation_compare}
\end{table*}
\endgroup


We sample triplets of frames in the reference video to train our pose-aware video blending network. Given a target frame. e.g. frame $i$, in the reference video to synthesize, we randomly sample two other nearby frames indexing $i-k_0$ and $i+k_1$, $k_0, k_1 \in [1, 8]$ as inputs to the network. The corresponding blending weight $t$ could be computed as ${k_1}/{(k_1 + k_2)}$ as well. We train the entire network end-to-end with losses defined to better estimate the flows and reconstruct the final image. We first have L1 reconstruction loss $L_{rec}$ and perceptual loss $L_{per}$ between synthesized image $\hat{I}_t$ and $I_t$. 

\begin{align}
    L_{rec} &= \L_1 (I_t, \hat{I}_t) \\
    L_{per} &= \L_1 (\phi(I_t), \phi(\hat{I}_t))
\end{align}

We also adopt L1 reconstruction loss $\L^{b}_{rec}$ for the deep feature $x''_0$ and $x''_1$ after they are passed through the generation network $G$.

\begin{equation}
    L^{b}_{rec} \&= \L_1 (I_t, G(x''_i)) + \L_1 (I_t, G(x''j0))
\end{equation}

We also have additional warping loss $L_{warp}$ by measuring the L1 difference between target image and the source images $I_i$ after being warped through $F^m_{t\to i}$ and $F^o_{t\to i}$ . 

\begin{align}
\begin{split}
    L^{m}_{warp} &= \L_1 (I_t, \W(I_i, F^m_{t\to i})) + \\
    &\ \ \ \ \ \ \ \ \ \ \L_1 (I_t, \W(I_j, F^m_{t\to j})) \\
     L^{o}_{warp} &= \L_1 (I_t, \W(\W(I_i, F^m_{t\to i}), F^o_{t\to i})) + \\
    &\ \ \ \ \ \ \ \ \ \ \L_1 (I_t, \W(\W(I_j, F^m_{t\to j}), F^o_{t\to j}))
\end{split}
\end{align}
where $\W(I, F)$ indicates applying backward warping flow $F$ on image $I$.

Finally, we follow \cite{jiang2018super} to have a smoothness loss for the optical flow filed as $L_{sm}$. 

\begin{equation}
    L_{sm} \&= ||\nabla F^{o}_{t\to i}||_1 + ||\nabla F^{o}_{t\to j}||_1
\end{equation}

The overall loss $\L$ is defined as the weighted sum of all losses defined above.

\begin{align}
\begin{split}
    \L = \L_{rec} + \lambda_{p}& \L_{per} + \lambda_b \L^b_{rec} + \\
    &\lambda_w (\L^m_{warp} + \L^o_{warp}) + \lambda_s \L_{sm}
\end{split}
\end{align}
The weights have been set empirically using the validation set
as $\lambda_{p}=0.01,\ \lambda_b=0.25,\ \lambda_w=0.25,\ \lambda_s=0.01$.


